Binarised Regression with Instance-Varying Costs: Evaluation using Impact Curves

Many evaluation methods exist, each for a particular prediction task, and there are a number of prediction tasks commonly performed including classification and regression. In binarised regression, binary decisions are generated from a learned regression model (or real-valued dependent variable), which is useful when the division between instances that should be predicted positive or negative depends on the utility. For example, in mining, the boundary between a valuable rock and a waste rock depends on the market price of various metals, which varies with time. This paper proposes impact curves to evaluate binarised regression with instance-varying costs, where some instances are much worse to be classified as positive (or negative) than other instances; e.g., it is much worse to throw away a high-grade gold rock than a medium-grade copper-ore rock, even if the mine wishes to keep both because both are profitable. We show how to construct an impact curve for a variety of domains, including examples from healthcare, mining, and entertainment. Impact curves optimize binary decisions across all utilities of the chosen utility function, identify the conditions where one model may be favoured over another, and quantitatively assess improvement between competing models.

==> tex_files/ack.tex <==
We would like to thank MineSense Technologies Ltd.\texttrademark\ 
for use of their sensor datasets.
%
We would also like to thank
Carol Ann McDevitt, Andrew Bamber, Iain McLean, and David Munoz Paniagua
for providing feedback and suggestions
in the development of Impact Curves.


==> tex_files/paper_draft.tex <==
\if 0
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Apple Sorting Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPLES EXAMPLE
As a toy example, suppose Apple Producer Company is sorting apples based on quality.
%
The actual quality is a continuum.
%
Apples that are completely bruised or mouldy are much worse to accept
than apples that are just barely below the threshold of an acceptable apple.

%
Apple Producer Company has 2 decision algorithms availabe to them
that have been trained on a training set 
and now are being tested on 4 apples.
%
The algorithms produce a quality prediction for each apple.
Figure \ref{fig:apples_1} and Figure \ref{fig:apples_2}
show the 4 apples
with the actual market value on the y-axis
and the predicted quality on the x-axis
for decision algorithms A1 and A2 respectively (Alg. A1, Alg. A2).

Suppose it costs Apple Producer Company 2 units to process every accepted apple,
and 0 units for every rejected apple.
%
Units may be dollars or any other unit of interest.
%
The operating profit for accepting an apple with market value of 5 is
5 less processing costs: $5 - 2 = 3$ units.
%
In Alg. A1,
setting the decision threshold to 40 yields a net profit of 5 (see Table \ref{tbl:alg1}).
%
In Alg. A2, a decision threshold of 40 would produce a net profit of 3 units,
but we can set the decision threshold to 20 instead to produce a net profit of 4
(see Table \ref{tbl:alg2}.


\begin{figure}[ht!] 
 \begin{center}
   % \includegraphics[width=0.88\linewidth]{fig/apples_1.svg}
	\includesvg[width=1\linewidth]{fig/apples_1}
   \caption{\label{fig:apples_1}
   Predicting apple quality using Alg. A1
 }
 \end{center}
\end{figure}

\begin{table}[htb]
\centering
\caption{Profit for Apple Sorting with Alg. A1, threshold=40}
\label{tbl:alg1}
\begin{tabular}{@{}lllll@{}}
\textbf{Alg. A1} \\
\toprule
Apple & Actual Market Value & Accepted? & Cost & Net \\ \midrule
\#1   & 0                   & No        & 0    & 0          \\
\#2   & 1                   & No        & 0    & 0          \\
\#3   & 4                   & Yes       & 2    & 2          \\
\#4   & 5                   & Yes       & 2    & 3          \\ \midrule
Total &                     &           &      & 5          \\ \bottomrule
\end{tabular}
\end{table}

\begin{figure}[ht!] 
 \begin{center}
	\includesvg[width=1\linewidth]{fig/apples_2}
   \caption{\label{fig:apples_2}
   Predicting apple quality using Alg. A2
 }
 \end{center}
\end{figure}

\begin{table}[htb]
\centering
\caption{Profit for Apple Sorting with Alg. A2, threshold=20}
\label{tbl:alg2}
\begin{tabular}{@{}lllll@{}}
\textbf{Alg. A2} \\
\toprule
Apple & Actual Market Value & Accepted? & Cost & Net \\ \midrule
\#1   & 0                   & No        & 0    & 0          \\
\#2   & 1                   & Yes       & 2    & -1         \\
\#3   & 4                   & Yes       & 2    & 2          \\
\#4   & 5                   & Yes       & 2    & 3          \\ \midrule
Total &                     &           &      & 4          \\ \bottomrule
\end{tabular}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Desiderata}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A representation of sorting performance should have the following qualities:
\begin{enumerate}
	\item Be simple to use and understandable by domain experts.
	\item Have enough information to guide the modelling process.
	\item Capture the relative value of each instance, where value is continuous.
	\item Clearly plot impact spanning a range of costs.
	%\item Incorporate the effects of a continuous actual.
	\item Convey if a prediction algorithm is worth using compared to a trivial prediction.
	\item Convey which of two prediction algorithms performs better.
	\item Show if one prediction algorithm is always better than another, in which case it is said to dominate.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Impact Curves}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In an impact curve, each instance has some continuous quantity that is of interest.
%
%The \textbf{actual} amount of this quantity has value associated with it.
%
% A decision algorithm creates a \textbf{prediction} for each instance, 
% and takes as input a decision threshold used to decide for each instance 
% whether to \textbf{accept} it or \textbf{reject} it
% (i.e. classify as positive or negative).
% A decision algorithm decides for each instance 
% whether to \textbf{accept} it or \textbf{reject} it
% (i.e. classify as positive or negative).
%
% We don't require access to the prediction;
% the prediction algorithm may be a black box that decides to either accept or reject each instance based on the decision threshold.
%
% We assume the decision algorithm has a parameter, or decision threshold,
% such that as the decision threshold increases, 
% the number of rejected instances also increases and the number of accepted instances decreases.
% i.e. monotonic decision threshold as function of number of instances

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if 0
	\subsection{Impact Definition}

	%%% IN OUR EXAMPLE
	In our apple sorting example, 
	the actual monotonically increases with decision threshold.
	%
	% and further, 
	% the actual, prediction, and decision threshold are in the same domain. 
	%
	The apple decision algorithm accepts an instance
	if its prediction of quality exceeds the decision threshold
	and rejects it otherwise.
	% 
	%
	The actual and decision threshold are not required to be in the same domain.
	% \matt{I believe this implies that the actual doesnt have to be a monotonic function of decision threshold, right?}

	%%% IMPACT
	We assume the accepted instances contribute value, or profit, whereas the rejected instances are discarded.
	There is a cost for every rejected instance 
	and a profit, or utility, for every accepted instance.
	%
	We define the total value of a set of decisions as a summation of the profit and costs over all instances which we call \textbf{impact}:

	% \matt{Formula version 1 $\rightarrow$}

	% \begin{equation}
	% \label{eq:impact}
	% impact = \sum_{i \in X}{\alpha v_i {\mathbb{I}(+_i)} - (c_a {\mathbb{I}(+_i)} + c_r {\mathbb{I}(-_i)})}
	% \end{equation}

	% where
	% $X$ is the set of instances,
	% $v_i$ is the actual value of the quantity of interest for instance $i$,
	% $\mathbb{I}(+_i)$ indicates 1 if the class of instance $i$ is positive and 0 if negative,
	% $\mathbb{I}(-_i)$ indicates 0 if the class of instance $i$ is positive and 1 if negative,
	% $c_{a}$ is the cost of processing one positive instance,
	% $c_{r}$ is the cost of processing one negative instance,
	% and
	% $\alpha$ is the value of 1 unit of the actual quantity
	% .


	\begin{equation}
	\label{eq:impactUtility}
	impact = \sum_{i \in A}{u^{+}(v_i)} - \sum_{i \in R}{u^{-}(v_i)}
	\end{equation}

	where 
	$A$ is the set of accepted instances,
	$R$ is the set of rejected instances,
	$v_i$ is the actual value of the quantity of interest for instance $i$,
	$u^{+}(v_i)$ is the utility of a positive instance,
	and
	$u^{-}(v_i)$ is the utility of a negative instance.
	%
	%%% TEST SET
	We assume the prediction algorithm is operating on a test set.
	% TODO: but if you want to CV, then you can optimize threshold
	%
	%

\fi


%%%%%%%%%%%%%%%%%%%%
\newif\ifLONGIMPACT
\LONGIMPACTfalse % set to true to use the long description, false to use short version
%%%%%%%%%%%%%%%%%%%%

\subsection{Impact Details}
In our application, 
the utility of accepting an instance is the actual of each instance multiplied
by a constant, $\alpha$, minus the cost of accepting one instance,
and the utility of rejecting an instance is simply the cost of rejecting one instance:

\begin{equation}
\label{eq:impact}
impact = \sum_{i \in A}{\left(\alpha v_i - c_a\right)} - \sum_{i \in R} c_r
\end{equation}

where 
$A$ is the set of accepted instances,
$R$ is the set of rejected instances,
$v_i$ is the actual of instance $i$,
$c_{a}$ is the processing cost of accepting an instance,
$c_{r}$ is the cost of rejecting an instance,
and
$\alpha$ is the multiplier relating profit to actual.
%
%
Impact (Eq. \ref{eq:impact}) has 3 parameters, 
but there is only 1 degree of freedom which determines the shape of the curve.
%
We reduce Eq. \ref{eq:impact} down to 1 parameter:

\ifLONGIMPACT {
	\begin{table}[htb]
	\centering
		\label{tbl:notation}
		\begin{tabular}{@{}ll@{}}
		\textbf{Notation} \\
		\toprule
		Symbol & Meaning \\ \midrule
		$I(t)$ & impact of decision algorithm as a function \\ & of threshold $t$ \\
		$\tilde{I}(t)$ & impact function arbitrarily scaled and shifted \\
		$\dot{\tilde{I}}(t)$ & impact function normalized to between 0 and 1 \\
		$X$ & all instances \\
		$A(t)$ & decision algorithm's set of accepted instances \\ & given threshold $t$ \\
		$R(t)$ & decision algorithm's set of rejected instances \\ & given threshold $t$ \\
		$n$ & number of instances in $X$ \\
		$|A(t)|$ & number of accepted instances in $A(t)$ \\
		$|R(t)|$ & number of rejected instances in $R(t)$ \\
		$\alpha$ & value of 1 unit of the actual quantity \\
		$c_a$ & cost of accepting one instance \\
		$c_r$ & cost of rejecting one instance \\
		$v_i$ & actual value of the quantity of interest for instance $i$ \\ \bottomrule
		\end{tabular}
	\end{table}

	\begin{align}
		I(t) &= \sum_{i \in A(t)}\left(\alpha v_i - c_a\right) - \sum_{i \in R(t)} c_r
		\\
		&= \sum_{i \in A(t)}\left(\alpha v_i - c_a\right) - |R(t)| c_r
		\nonumber
		\\
		&= \sum_{i \in A(t)}\left(\alpha v_i\right) - |A(t)| c_a - |R(t)| c_r
		\nonumber
		\\
		&= \sum_{i \in A(t)}\left(\alpha v_i\right) - |A(t)| c_a - |R(t)| c_r - n c_r + n c_r
		\nonumber
		\\
		&= \sum_{i \in A(t)}\left(\alpha v_i\right) - |A(t)| (c_a - c_r) - |R(t)| (c_r - c_r) - n c_r
		\nonumber
		\\
		&= \sum_{i \in A(t)}\left(\alpha v_i\right) - |A(t)| (c_a - c_r) - n c_r
		\nonumber
		\\
		&= \alpha \sum_{i \in A(t)} v_i - |A(t)| (c_a - c_r) - n c_r
		\nonumber
		\\
		&= \left(c_a - c_r\right) \left( \frac{\alpha}{c_a - c_r} \sum_{i \in A(t)} v_i - |A(t)|\right) - n c_r
		\label{eq:impact2}
	\end{align}

	Notice that only the term inside the large parentheses depends on $t$, 
	therefore the shape of the function with respect to $t$ only depends on this term:

	\begin{align}
		\tilde{I}(t) &= \frac{\alpha}{c_a - c_r} \sum_{i \in A(t)} v_i - |A(t)|
	\end{align}

	which has one degree of freedom relating to the associated costs and value.
	Let $\beta$ be the ratio of profit to difference in processing costs:

	\begin{equation}
	\label{eq:tildeImpact}
		\tilde{I}(t) = \beta \sum_{i \in A(t)} v_i - |A(t)|
	\end{equation}

	When the cost of rejecting an instance is zero, 
	then $\beta$ is simply the ratio of profit to cost of accepting an instance:
	\begin{equation}
		\beta = \frac{\alpha}{c_{a}}
	\end{equation}
	%
	If processing costs double, $\beta$ is halved. If profit doubles, $\beta$ is doubled.
	%
	%Figure \ref{fig:apple_alg_cost1} is an Impact Curve where $\beta$ is $1$.

	\begin{proposition}
	Given two decision algorithms, $_1$ and $_2$,
	if $I_1(t) < I_2(t)$ then $\tilde{I}_1(t) < \tilde{I}_2(t)$.
	And similarly for $<$, $\le$, $>$, $\ge$, $\ne$, $=$.
	\end{proposition}

	\begin{proof}

	Let $I(t) = m \tilde{I}(t) + b$
	where $m = (c_a - c_r)$,
	and $b = -n c_r$.
		
	\begin{align}
		I_1(t) &< I_2(t)
		\nonumber \\
		m\ \tilde{I}_1(t) + b &< m\ \tilde{I}_2(t) + b
		\nonumber \\
		m\ \tilde{I}_1(t) + b - b &< m\ \tilde{I}_2(t) + b - b
		\nonumber \\
		m\ \tilde{I}_1(t) &< m\ \tilde{I}_2(t)
		\nonumber \\
		\frac{m}{m}\ \tilde{I}_1(t) &< \frac{m}{m}\ \tilde{I}_2(t)
		\nonumber \\
		\tilde{I}_1(t) &< \tilde{I}_2(t)
		\nonumber
	\end{align}

	% \begin{itemize}
	% 	\item $I_1(t)$: impact of decision algorithm \#1
	% 	\item $I_2(t)$: impact of decision algorithm \#2
	% \end{itemize}

	\end{proof}
	% \hfill$\square$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
} \else {
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{equation}
		I(t) = \left(c_a - c_r\right) \left( \beta \sum_{i \in A(t)} v_i - |A(t)|\right) - n c_r
		\label{eq:impact2}
	\end{equation}

	where
	$\beta$ is $\frac{\alpha}{c_a - c_r}$ which is the ratio of profit to difference in processing costs,
	$I(t)$ is the impact of a decision algorithm as a function of threshold $t$,
	$A(t)$ is decision algorithm's set of accepted instances given threshold $t$,
	$|A(t)|$ is number of accepted instances,
	$n$ is the total number of instances,
	and
	$\alpha$ is value of 1 unit of the actual quantity.
	Notice that only the term inside the large parentheses depends on $t$, 
	therefore the shape of the function with respect to $t$ only depends on $\beta$.
} \fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Normalization}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifLONGNORM
\LONGNORMfalse % set to true to use the long description of normalization, false to use short version

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifLONGNORM {
	Impact can be infinitely high because $\beta$ can be infinitely high.
	%
	For convenience in plotting, we can normalize the range to between $-1$ and $1$
	by dividing impact, $\tilde{I}$, by the range.

	\begin{equation}
	\label{eq:normalized}
		\dot{\tilde{I}}(t) = 
		\frac{
			\tilde{I}(t)
		}{
			maxImpact - minImpact
		}
	\end{equation}

	$minImpact$ is found by taking the limit of $\tilde{I}(t)$ as $\beta$ approaches zero:

	\begin{align}
		minImpact &= \lim_{\beta \to 0}\ \ \beta \sum_{i \in X} v_i - |X|
		\nonumber \\
		&= 0 - |X|
		\nonumber \\
		&= -|X|
	\end{align}

	$maxImpact$ is found by taking the limit of $\tilde{I}(t)$ as $\beta$ approaches infinity:

	\begin{align}
		maxImpact &= \lim_{\beta \to \inf}\ \ \beta \sum_{i \in X} v_i - |X|
		\label{eq:maxImpact_1} \\
		&= \lim_{\beta \to \inf}\ \ \sum_{i \in X} v_i - \frac{1}{\beta} |X|
		\label{eq:maxImpact_2} \\
		&= \sum_{i \in X} v_i - \lim_{\beta \to \inf}\ \ \frac{1}{\beta} |X|
		\nonumber \\
		&= \sum_{i \in X} v_i - 0
		\nonumber \\
		&= \sum_{i \in X} v_i
	\end{align}

	The step from Eq. \ref{eq:maxImpact_1} to \ref{eq:maxImpact_2} is possible because
	in Eq. \ref{eq:impact2} we could have factored $\alpha$ instead of $(c_a - c_r)$.
	%
	Substituting $maxImpact$ and $minImpact$ into Eq. \ref{eq:normalized} we get:

	\begin{align}
		\dot{\tilde{I}}(t) &= 
		\frac{
			\tilde{I}(t)
		}{
			\left( \sum_{i \in X} v_i \right) - \left( -|X| \right)
		}
		\nonumber \\
		&= \frac{
			\tilde{I}(t)
		}{
			\sum_{i \in X} v_i + |X|
		}
	\end{align}
} \else {
	Impact can be infinitely high because $\beta$ can be infinitely high.
	%
	For convenience in plotting, we can normalize the range to between $-1$ and $1$
	by dividing impact by the range:

	\begin{align}
	\label{eq:normalized}
		\dot{I}(t) &= 
		\frac{
			\beta \sum_{i \in A(t)} v_i - |A(t)|
		}{
			\sum_{i \in X} v_i + |X|
		}
	\end{align}

	where $\dot{I}(t)$ is normalized impact,
	and $X$ is the set of all instances.
} \fi

% For the remainder of the paper we plot normalized impact, $\dot{\tilde{I}}(t)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Plotting an Impact Curve}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% IMPACT SENSITIVITY
As decision threshold varies in the apple sorting example
we get varying values for impact.
%
For instance, Table \ref{tbl:alg1} is when $\beta=0.5$, or $\alpha=1$, $c_a=2$, and $c_r=0$.
The impact across thresholds is shown in Figure \ref{fig:apple_alg1_betaHalf}.
%
This shows the sensitivity of the algorithm to impact.

\if 0
\begin{figure}[htbp] 
 \begin{center}
 \includesvg[width=1\linewidth]{fig/apple_alg1_betaHalf}
   \caption{
   \label{fig:apple_alg1_betaHalf}
   Impact sensitivity for Alg. A1 
   given that it costs 2 units
   to process every accepted apple.
 }
 \end{center}
\end{figure}
\fi

%%% IMPACT CURVE
As $\beta$ varies, we want to know the best impact achievable for each algorithm.
%
% An impact curve plots $max($\textit{impact}$)$ on the y-axis versus $\beta$ on the x-axis,
\matt{Actual it's the max impact over decision thresholds, removed for simplicity}%
%
An impact curve plots \textit{impact} on the y-axis versus $\beta$ on the x-axis,
where \textit{impact} 
% is one of  $I(t)$, $\tilde{I}(t)$, or $\dot{\tilde{I}}(t)$ (Eq. \ref{eq:impact2}, \ref{eq:tildeImpact}, \ref{eq:normalized}).
is $I(t)$ or $\dot{I}(t)$ (Eq. \ref{eq:impact2}, \ref{eq:normalized}).
%
The shape of the impact curve will remain the same regardless of which form of \textit{impact} you choose.
%
For example, the apple sorting example can be seen in Figure \ref{fig:apple_ImpactVsBeta}.

\if 0
\begin{figure}[htbp] 
 \begin{center}
 \includesvg[width=1\linewidth]{fig/apple_ImpactVsBeta}
   \caption{
   \label{fig:apple_ImpactVsBeta}
   Impact curve for apple sorting example.
 }
 \end{center}
\end{figure}
\fi

%%% IMPACT IMPROVEMENT
We are usually only interested in how much improvement is gained
from sorting versus trivially accepting or rejecting all the instances.
Therefore, an impact improvement curve
%
plots impact minus the impact of trivially accepting or rejecting all the instances (whichever is higher).

% plots $\Delta max($impact$)$ on the y-axis versus $\beta$ on the x-axis,
% as shown in Figure \ref{fig:apple_ImpactImprovementVsBeta} for the apple sorting example,
% where $\Delta max($impact$)$ is as follows:

% \begin{equation}
% 	\Delta max(impact) = \max_{t \in T}{I(t)} - trivial
% \end{equation}

% where 
% $T$ is the set of thresholds of interest to the modeller,
% and
% $trivial$ is the impact of either accepting or rejecting all the instances, whichever is higher.

\if 0
\begin{figure}[htbp] 
 \begin{center}
 \includesvg[width=1\linewidth]{fig/apple_ImpactImprovementVsBeta}
   \caption{
   \label{fig:apple_ImpactImprovementVsBeta}
   Impact improvement curve for apple decision algorithms A1 and A2.
 }
 \end{center}
\end{figure}
\fi

We now have the necessary information to determine which decision algorithm performs the best.
From Figure \ref{fig:apple_ImpactImprovementVsBeta} we see that Alg. A1 is better than Alg. A2 for all values of $\beta$.
%
It can be said the Alg. A1 dominates Alg. A2, which means that in practice we will choose to use Alg. A1 and not Alg. A2 regardless of $\beta$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Limitations and Future Work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\matt{Similarly, choosing the max impact at each $\beta$ is optimistic; cross-validation should be considered.}%
%
%
%Impact can be extended to non-linear profit functions.
%
%
%
%Impact curves only visualize one parameter referred to as decision threshold.
%This could expanded to multiple parameters,
%and further to multi-dimensional predictions.
% Often  and it should be in the same domain as prediction (not really required though...)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Application to Mining}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
% Define True Grade Cutoff
Grade cutoff is used as the decision threshold in Impact Curves.
%
% The grade cutoff is specified by the mine and reflects what they believe is their break-even point. 
% %
% That is, the point at which it is no longer economical to accept for processing the samples below the cutoff.
% %
% Grade cutoff is an expression of the mine's utility around which there is uncertainty that the value is estimated correctly and which is open to change in the future.



% Define sorting algorithm's grade cutoff
% Every sorting algorithm also has a configurable threshold parameter. For example, if false negatives are highly undesirable then we may set the algorithm threshold lower than the grade threshold to provide some assurance that samples near the true grade cutoff won't be misclassified.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impact Curves for Mining Dataset}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The cost of processing is unknown as is the market value for copper
% because these values fluctuate and are dependent on mine-specific information.
% %
% Nonetheless, we can plot Impact Curves for a variety of costs to see under
% what circumstances which algorithm performs better.

In this application we are sorting barrels of rocks,
where one sample is a whole barrel.
%
A preliminary dataset has been collected consisting of 122 samples.
%
We assume the weight of each sample is equal.
%
%%% RELATE TO UTILITY & IMPACT
%
The utility of accepting a sample is the actual grade of copper of the sample multiplied by a positive constant ($\alpha$)
minus the cost of processing an accepted sample.
%
The utility of rejecting a sample is simply the cost of throwing away the sample,
which for this application is 0.


%
At the time of writing, the cost of 100\% copper with the same
weight as a sample is \$816.77 USD. 
%
For one mine, the processing cost for accepting a sample may be \$5.45
and the cost for rejecting a sample is very close to \$0.
Therefore, $\beta = \frac{816.77 / 100}{5.45 - 0} = 1.5$.
%
Figure \ref{fig:MTL_LD_bsn_lasso} shows the impact sensitivity 
of two decision algorithms
on the 122 samples for $\beta = 1.5$.

Figure \ref{fig:MTL_LD_bsn_lasso_ImpactVsBeta} shows the impact curves for
the two decision algorithms.
%
Many mines don't employ any sorting of this kind,
therefore the improvement is between the best decision algorithm and trivially accepting or rejecting all the samples.
%
Figure \ref{fig:MTL_LD_bsn_lasso_ImpactImprovementVsBeta} shows the impact improvement relative
to the best trivial sorting method.


\if 0
\begin{figure}[htbp] 
 \begin{center}
   \includesvg[width=1\linewidth]{fig/MTL_LD_bsn_lasso_I} % has annotations
	% \includesvg[width=1\linewidth]{fig/MTL_LD_bsn_lasso} % no annotations
   \caption{\label{fig:MTL_LD_bsn_lasso}
   Impact sensitivity curves for sorting rock samples based on predicted copper grade.
   Alg. C1 max impact is \$195.15, Alg. C2 max impact is \$188.24,
   and the impact of accepting all samples is \$116.51.
 }
 \end{center}
\end{figure} 

\begin{figure}[htbp] 
 \begin{center}
	\includesvg[width=1\linewidth]{fig/MTL_LD_bsn_lasso_ImpactVsBeta}
   \caption{\label{fig:MTL_LD_bsn_lasso_ImpactVsBeta}
   Impact curve for sorting rock samples based on predicted grade.
 }
 \end{center}
\end{figure} 

\begin{figure}[htbp] 
 \begin{center}
	\includesvg[width=1\linewidth]{fig/MTL_LD_bsn_lasso_ImpactImprovementVsBeta}
   \caption{\label{fig:MTL_LD_bsn_lasso_ImpactImprovementVsBeta}
   Impact improvement curve for sorting rock samples based on predicted grade.
 }
 \end{center}
\end{figure} 
\fi
%%%%%%%%


%%%TODO replace the section below

% Alg. C1 performed the best as seen in Figure \ref{fig:MTL_LD_bsn_lasso} with an impact
% of \$195.15.
% %
% The improvement over accepting all samples is $\$195.15 - \$116.51 = \$78.65$ per 122 runs,
% which is 19.4 tonnes of rock.
% %
% Per tonne the improvement is $\$78.65 / 19.4 = \$4.05$.

% Chile produced 2.43 million tonnes of copper in a 5 month period in 2015,
% translating to roughly 310 million tonnes of rock.
% %
% Employing Alg. C1 is all of Chile would result in $\$4.05 * 310$ million $ =  \$1,257,457,498.38$,
% or \$1.26 billion dollars more profit.
% %
% The improvement of Alg. C1 over Alg. C2 would result in \$110 million dollars more profit.

